DeepFlow: Abnormal Traffic Flow Detection Using Siamese Networks

Nowadays, many cities are equipped with surveillance systems and traffic control centers to monitor vehicular traffic for road safety and efficiency. The monitoring process is mostly done manually which is inefficient and expensive. In recent years, several data-driven solutions have been proposed in the literature to automatically analyze traffic flow data using machine learning techniques. However, existing solutions require large and comprehensive datasets for training which are not readily available, thus limiting their application. In this paper, we develop a traffic anomaly detection system, referred to as DeepFlow, based on Siamese neural networks, which are suitable in scenarios where only small datasets are available for training. Our model can detect abnormal traffic flows by analyzing the trajectory data collected from the vehicles in a fleet. To evaluate DeepFlow, we use realistic vehicular traffic simulations in SUMO. Our results show that DeepFlow detects abnormal traffic patterns with an F1 score of 78%, while outperforming other existing approaches including: Dynamic Time Warping (DTW), Global Alignment Kernels (GAK), and iForest.

==> com/centcap.tex <==

\usepackage{varwidth}
\DeclareCaptionFormat{myformat}{%
  % #1: label (e.g. "Table 1")
  % #2: separator (e.g. ": ")
  % #3: caption text
  \begin{varwidth}{\linewidth}%
    \centering
    #1#2#3%
  \end{varwidth}%
}
\captionsetup{format=myformat}


==> com/centfig.tex <==

% for centered figure captions in journal mode
\makeatletter
\long\def\@makecaption#1#2{\ifx\@captype\@IEEEtablestring%
\footnotesize\begin{center}{\normalfont\footnotesize #1}\\
{\normalfont\footnotesize\scshape #2}\end{center}%
\@IEEEtablecaptionsepspace \else \@IEEEfigurecaptionsepspace
\setbox\@tempboxa\hbox{\normalfont\footnotesize {#1.}~~ #2}%
\ifdim \wd\@tempboxa >\hsize%
\setbox\@tempboxa\hbox{\normalfont\footnotesize {#1.}~~ }%
\parbox[t]{\hsize}{\normalfont\footnotesize \noindent\unhbox\@tempboxa#2}%
\else \hbox
to\hsize{\normalfont\footnotesize\hfil\box\@tempboxa\hfil}\fi\fi}
\makeatother 

==> com/margins.tex <==

\setlength{\oddsidemargin}{0.5in}
\setlength{\evensidemargin}{0.5in}
\setlength{\textwidth}{5in}


==> com/mathdefs.tex <==

\newcommand{\pr}[1]{\mathbb{P}\left\{#1\right\}}
\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\V}[1]{\mathrm{Var}\left(#1\right)}
\newcommand{\ol}[1]{\overline{#1}}
\newcommand{\mx}[1]{\ensuremath{\mathbf{#1}}}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\ang}[1]{\langle #1 \rangle}


==> com/pagenum.tex <==

\makeatletter
\def\ps@headings{%
\def\@oddhead{\mbox{}\scriptsize\rightmark \hfil \thepage}%
\def\@evenhead{\scriptsize\thepage \hfil \leftmark\mbox{}}%
\def\@oddfoot{}%
\def\@evenfoot{}}
\makeatother 
\pagestyle{headings}


==> com/titlespace.tex <==

\IEEEoverridecommandlockouts
\IEEEaftertitletext{\vspace{-0.3cm}}
\bstctlcite{IEEEexample:BSTcontrol} 


==> tex/references.tex <==

    \begin{thebibliography}{00}

        \bibitem{R1} M. Zhang, C. Chen, T. Wo, T. Xie, M. Z. A. Bhuiyan and X. Lin, "SafeDrive: Online Driving Anomaly Detection From Large-Scale Vehicle Data," in IEEE Transactions on Industrial Informatics, vol. 13, no. 4, pp. 2087-2096, Aug. 2017.

        \bibitem{R2} Hao Wu, Weiwei Sun, and Baihua Zheng. 2017. A Fast Trajectory Outlier Detection Approach via Driving Behavior Modeling. In Proceedings of the 2017 ACM on Conference on Information and Knowledge Management (CIKM '17). Association for Computing Machinery, New York, NY, USA, 837–846. DOI:https://doi.org/10.1145/3132847.3132933

        \bibitem{R4} H. Oikawa, T. Nishida, R. Sakamoto, H. Matsutani and M. Kondo, "Fast Semi-Supervised Anomaly Detection of Drivers’ Behavior using Online Sequential Extreme Learning Machine," 2020 IEEE 23rd International Conference on Intelligent Transportation Systems (ITSC), Rhodes, Greece, 2020, pp. 1-8, doi: 10.1109/ITSC45102.2020.9294659.

        \bibitem{R3} M. Matousek, M. Yassin, A. Al-Momani, R. van der Heijden and F. Kargl, "Robust Detection of Anomalous Driving Behavior," 2018 IEEE 87th Vehicular Technology Conference (VTC Spring), Porto, Portugal, 2018, pp. 1-5, doi: 10.1109/VTCSpring.2018.8417777.

        \bibitem{R5} L. Zhang, L. Yan, Y. Fang, X. Fang and X. Huang, "A Machine Learning-Based Defensive Alerting System Against Reckless Driving in Vehicular Networks," in IEEE Transactions on Vehicular Technology, vol. 68, no. 12, pp. 12227-12238, Dec. 2019, doi: 10.1109/TVT.2019.2945398.

        \bibitem{R6} S. Ucar, C. Patnayak, P. Oza, B. Hoh and K. Oguchi, "Management of Anomalous Driving Behavior," 2019 IEEE Vehicular Networking Conference (VNC), Los Angeles, CA, USA, 2019, pp. 1-4, doi: 10.1109/VNC48660.2019.9062814.

        \bibitem{R7} A. S. Yuksel & S. Atmaca (2020) Driver’s black box: a system for driver risk assessment using machine learning and fuzzy logic, Journal of Intelligent Transportation Systems, DOI: 10.1080/15472450.2020.1852083

        \bibitem{R8} “Dynamic Time Warping,” in Information Retrieval for Music and Motion, Berlin, Heidelberg: Springer Berlin Heidelberg, 2007, pp. 69–84.

        \bibitem{R9} Cuturi, Marco. (2011). Fast Global Alignment Kernels.. Proceedings of the 28th International Conference on Machine Learning, ICML 2011. 929-936.

        \bibitem{R10} Towards Zero: The Safest Roads in the World

        \bibitem{R11} Pablo Alvarez Lopez, Michael Behrisch, Laura Bieker-Walz, Jakob Erdmann, Yun-Pang Flötteröd, Robert Hilbrich, Leonhard Lücken, Johannes Rummel, Peter Wagner, and Evamarie Wießner. IEEE Intelligent Transportation Systems Conference (ITSC), 2018.

        \bibitem{R12}  A. Wegener, M. Piórkowski, M. Raya, H. Hellbrück, S. Fischer and J. P. Hubaux, "Traci: An interface for coupling road traffic and network simulators", Proceedings of the 11th Communications and Networking Simulation Symposium CNS '08, pp. 155-163, 2008.

    \end{thebibliography}
